Stallings folds for CAT(0) cube complexes and quasiconvex subgroups

We describe a higher dimensional analogue of the Stallings folding sequence for group actions on CAT(0) cube complexes. We use it to give a characterization of quasiconvex subgroups of hyperbolic groups which act properly co-compactly on CAT(0) cube complexes via finiteness properties of their hyperplane stabilizers.

==> cocompactness2.tex <==
% !TeX root = main.tex

%\section{Coboundedness}
We first show that performing a \bla preserves coboundedness.

\begin{lemma} \label{cobounded}
Let $\gp{G}$ be a group acting coboundedly on a \CCC $\CC{X}$. Let $\CC{Y}$ be a \CCC obtained by a $\gp{G}$-\bla $f$ of $X$. Then the action of $\gp{G}$ on $\CC{Y}$ is cobounded.
\end{lemma}


\begin{proof}
From Lemma \ref{AMtoCCCmap}, the map $F:  \CC{X} \rightarrow \CC{Y}$ is distance non-increasing. It is thus sufficient to prove that $\CC{Y}$ is at bounded distance from the image of $F$. We are going to show that any maximal cube in  $\CC{Y}$ contains at least a vertex in the image.

For a maximal cube $\CCc{C}$ in $\CC{Y}$, we associate the vertex $\CCv{x}$ in $\CC{X}$ defined as the following ultrafilter. Denote by $S$ the set of non folded hyperplanes of $\CCc{C}$ and by $T$ the set of folded ones.

For each $\hyp k$ in $S$, there is only one preimage $\hyp h$ by $f$. We fix an arbitrary orientation for $\hyp h$.

For each $\hyp k$ in $T$, the set  $f^{-1}(\hyp{k})$ is a set of comparable hyperplanes such that none is in between any two other. We  can thus choose the orientation such that they all face one another.

For any other $\hyp{h}\in \Hyp{H}(\CC{X})$, $f(\hyp{h})$ is comparable with a hyperplane $\hyp k$ of $S$ or $T$. So we choose the orientation of $\hyp{h}$ toward an element of  $f^{-1}(\hyp k)$. Note that it does not depend on the chosen preimage, otherwise $\hyp{h}$ would be in between two hyperplanes folded onto $\hyp k$, and thus $f(\hyp{h})$ and $\hyp k$ would cross.

Let us first check that it defines an ultrafilter of $\CC{X}$. It is sufficient to check that the orientations on preimages of $S$ and $T$ are compatible.
First of all, as elements of $S$ are not folded and are pairwise crossing in $Y$, their unique preimages are pairwise crossing. So the chosen orientations are compatible for $S$.
Now take $\hyp k$ in $S\cup T$ and $\hyp k'\neq \hyp k$ in $T$. By assumption, the hyperplanes $\hyp k$ and $\hyp k'$ are crossing. So either there exists $\hyp h'$ in the preimage of $\hyp k'$ that is crossing $\hyp h$ a preimage of $\hyp k$. Then as any hyperplane in $f^{-1}(\hyp k)\cup f^{-1}(\hyp k')$ is oriented toward $\hyp h \cap \hyp h'$, any pair of preimages is oriented in a compatible way.
Or, (up to interchange the role $\hyp k$ and $\hyp k'$), there are two hyperplanes $\hyp h'$ and $\hyp h''$ in $f^{-1}(\hyp k')$ separated by an hyperplane $\hyp h\in f^{-1}(\hyp k)$. So $\hyp h'$ and $\hyp h''$ are oriented toward $\hyp h$, and $\hyp h$ is oriented toward one of $\hyp h'$ and $\hyp h''$. By construction any element in $f^{-1}(\hyp k)$ is oriented in direction of $\hyp h$ and elements $f^{-1}(\hyp k')$ are facing toward $\hyp h'$ and $\hyp h''$, and thus toward $\hyp h$. So each element of $f^{-1}(\hyp k)$ has a compatible orientation with any element of $f^{-1}(\hyp k')$.

Let us prove now that $F(\CCv{x})$ belongs to $\CCc{C}$. We have to show that any hyperplane $\hyp k$ not in $\CCc{C}$ is oriented toward a hyperplane of $\CCc{C}$ in the ultrafilter defined by $F(\CCv{x})$. Take the minimal hyperplane $\hyp h$ of $f^{-1}(\hyp k)$. By construction there exists  $\hyp k \in S\cup T$ such that $\hyp k$ and $\hyp k'$ are comparable his and the orientation in $\CCv{x}$ has been chosen toward some (thus any) lift $\hyp h'$ of $\hyp k'$. Hence the orientation of $\hyp k$ is toward  $\hyp k'$.

The $L_1$ distance between $\CC{Y}$ and the image of $F$ is bounded by the dimension of $\CC{Y}$.
\end{proof}

==> foldings2.tex <==
% !TeX root = main.tex

\section{Stallings foldings}

 We give in this section a definition for an equivalent of Stallings foldings in the case of higher dimensional \CCC. The goal of this section is to prove that a resolution can be decomposed as a finite sequence of elementary foldings.
 
Given a pocset $\Hs{H}$ endowed with an action of $G$, an \emph{\bla} is a quotient of the form $\Hs{H}/\hspace{-.15cm}\sim$ where $\sim$ is the minimal $G$-invariant and $\comp{}$-invariant equivalence relation generated by $\hs{h}_1\sim\hs{h}_2$ for two facing halfspaces.
The \emph{elementary folding} is a \bla compatible with $f:\Hs{H}\to\Hs{H}'$ a $G$-equivariant resolution of pocsets, that is, such that  $f(\hs{h}_1)=f(\hs{h}_2)$ and there is no pair of $\sim_f$-equivalent hyperplanes that separate $\hyp{h}_1$ and $\hyp{h}_2$.

\input{cocompactness2.tex}

\begin{lemma}
Let $f_0:\Hs{H}\to\Hs{H}'$ be a $G$-equivariant resolution. Let $\sim$ be an elementary folding as above. Then $\sim$ is an admissible equivalence relation and $f_1:\Hs{H}/\hspace{-.15cm}\sim\to\Hs{H}'$ is again a resolution.
\end{lemma}

\begin{proof}
By definition, the equivalence relation $\sim$ satisfies \ref{compinv}. To prove properties \ref{selfcomp} and \ref{welloriented} we simply observe that any class of $\sim$-equivalent hyperplanes are facing, for otherwise, the two folded hyperplanes are not minimal. Property \ref{selfcross} follows from the fact that the map $f_0$ is admissible, and thus if $\hyp{h}\pitchfork\hyp{k}$ then their images in $\Hs{H}'$ are distinct and in particular they are not equivalent.

We now show that $f_1$ is admissible. Since properties \ref{AMcompinv} and \ref{AMcompactible_image} clearly hold for $f_1$, we are left to show that $f_1$ satisfies properties \ref{AMcrossinghyps} and \ref{AMfacinghyps}.

Let $[\hyp{h}]\pitchfork[\hyp{k}]\in\Hs{H}/\hspace{-.15cm}\sim$ then either there exist representatives $\hyp{h}\pitchfork\hyp{k}\in\Hs{H}$ of $[\hyp{h}]$ and $[\hyp{k}]$ respectively, in which case they have distinct images because of property\ref{AMcrossinghyps} for $f_0$, or there exists some representative $\hyp{h}$ of $[\hyp{h}]$ that separates two representatives $\hyp{k}_1,\hyp{k}_2$ of $[\hyp{k}]$.
They are $\sim$-equivalent, and thus there exists a chain $\hyp{k}_1=\hyp{l}_1, \hyp{l}_2,\ldots,\hyp{l}_n=\hyp{k}_2$ such that each consecutive pair $\{\hyp{l}_i, \hyp{l}_{i+1}\}$ is of the form $\{g_i\hyp{h}_1,g_i\hyp{h}_2\}$ where $\hyp{h}_1$ and $\hyp{h}_2$ are the minimal hyperplanes that were folded in the elementary folding, and $g_i$ is some element of $G$.
Since $\hyp{h}$ separates $\hyp{k}_1,\hyp{k}_2$, and does not cross any lift of $[\hyp{k}]$, there is some $i$ for which $\hyp{h}$ separates $\hyp{l}_i,\hyp{l}_{i+1}$. Thus we may assume that $\hyp{k}_1,\hyp{k}_2$ are of the form $g\hyp{h}_1,g\hyp{h}_2$.
Now it easily follows that $f_1([\hyp{h}])\neq f_1([\hyp{k}])$ for otherwise we will get a contradiction to the minimality of $\hyp{h}_1$ and $\hyp{h}_2$.

To prove \ref{AMfacinghyps} it suffices to note that if two halfspaces  $[\hs{h}],[\hs{k}]\in\Hs{H}/\hspace{-.15cm}\sim$ are facing halfspaces, that satisfy $f_1([\hyp{h}])=f_1([\hyp{k}])$ and are minimal as hyperplanes among the other preimages of their image then so do their minimal representatives in $\Hs{H}$. Property \ref{AMfacinghyps} of $f_1$ follows from that of $f_0$.

We are left to show that the induced map $(\Hs{H}/\hspace{-.15cm}\sim)/\hspace{-.15cm}\sim_{f_1}\embedsin\Hs{H}'$. In fact we will prove that $(\Hs{H}/\hspace{-.15cm}\sim)/\hspace{-.15cm}\sim_{f_1}\simeq\Hs{H}/\hspace{-.15cm}\sim_{f_0}$ as pocsets, via the natural isomorphism $\left[ [\hs{h}]_\sim \right]_{\sim_{f_1}} \leftrightarrow [\hs{h}]_{\sim_{f_0}}$. This map is clearly a bijection, and the complementary operation is clearly preserved. We are left to show that this map is order preserving.

Let $[\hs{h}]_{\sim_{f_0}}<[\hs{k}]_{\sim_{f_0}}\in \Hs{H}/\hspace{-.15cm}\sim_{f_0}$, that is, any two representatives $\hs{h},\hs{k}$ of $[\hs{h}]_{\sim_{f_0}}, [\hs{k}]_{\sim_{f_0}}$ which are minimal as hyperplane representatives satisfy $\hs{h}<\hs{k}$. 

Now let $[[\hs{h}]_\sim]_{\sim_{f_1}}<[[\hs{k}]_\sim]_{\sim_{f_1}}\in (\Hs{H}/\hspace{-.15cm}\sim)/\hspace{-.15cm}\sim_{f_1}$, we show that the same condition as above holds.
Let $[\hs{h}]_\sim,[\hs{k}]_\sim$ be minimal representatives in $\Hs{H}/\hspace{-.15cm}\sim$ of $[[\hs{h}]_\sim]_{\sim_{f_1}},[[\hs{k}]_\sim]_{\sim_{f_1}}$ respectively among all hyperplane representatives, then by definition $[\hs{h}]_\sim<[\hs{k}]_\sim$.
Now, let $\hs{h}, \hs{k}$ be representatives in $\Hs{H}$ of $[\hs{h}]_\sim,[\hs{k}]_\sim$, which are minimal among all hyperplane representatives, then $\hs{h}<\hs{k}$. We are left to show that $\hyp{h},\hyp{k}$ are minimal among all hyperplane representatives of $[\hyp{h}]_{\sim_{f_0}},[\hyp{k}]_{\sim_{f_0}}$. Assume for contradiction that $\hyp{l}$ represents either $[\hyp{h}]_{\sim_{f_0}}$ or $[\hyp{k}]_{\sim_{f_0}}$, and separates $\hyp{h}$ and $\hyp{k}$. 
We have that non of the hyperplanes $[\hyp{h}]_\sim,[\hyp{k}]_\sim,[\hyp{l}]_\sim$ cross, as otherwise $[[\hs{h}]_\sim]_{\sim_{f_1}}\pitchfork[[\hs{k}]_\sim]_{\sim_{f_1}}$ in contradiction with the assumption. 
We thus claim that $[\hyp{l}]_\sim$ separates $[\hyp{h}]_\sim,[\hyp{k}]_\sim$, otherwise it is in $[\hs{k}]_\sim$ or in $[\comp{\hs{h}}]_\sim$, which leads to a contradiction to the minimality of $\hyp{h},\hyp{k}$ as hyperplane representatives of $[\hyp{h}]_{\sim_{f_0}},[\hyp{k}]_{\sim_{f_0}}$.
But now, we contradicted the minimality of $[\hyp{h}]_\sim,[\hyp{k}]_\sim$ among representatives of $[[\hs{h}]_\sim]_{\sim_{f_1}}<[[\hs{k}]_\sim]_{\sim_{f_1}}$, because $[[\hs{h}]_\sim]_{\sim_{f_1}}=[[\hs{l}]_\sim]_{\sim_{f_1}}$ or $[[\hs{k}]_\sim]_{\sim_{f_1}}=[[\hs{l}]_\sim]_{\sim_{f_1}}$.
\end{proof}

We obtain a decomposition of resolution as a finite sequence of elementary foldings.

\begin{proposition}\label{finite_folding}
Let $G$ be a group, let $\Hs{H},\Hs{H}'$ be $G$-pocsets, and let $f:\Hs{H}\to\Hs{H}'$ be a $G$-equivariant resolution. If $G$ acts cofinitely on the pocset $\Hs{H}$, and the $G$-stabilizers of hyperplanes in $\Hyp{H}'$ are finitely generated, then there exists a finite sequence of elementary foldings $$ \Hs{H}=\Hs{H}_0 \leadsto \Hs{H}_1 \leadsto \ldots \leadsto \Hs{H}_n=\Hs{H}/\hspace{-.15cm}\sim_f\embedsin\Hs{H}'$$
\end{proposition}

\begin{proof}
We first show that by a finite sequence of elementary foldings one can get $\Hs{H}_i$ such that $\Hs{H}_i/G\to\Hs{H}'/G$ is injective. If this map is not injective, choose two hyperplanes $\hyp{h},\hyp{k}$ such that $f(\hyp{h})=f(\hyp{k})$ but $\hyp{h}$ and $\hyp{k}$ belong to distinct $G$-orbits. Let $(\hyp{h},\hyp{k})$ be the collection of hyperplanes separating $\hyp{h}$ from $\hyp{k}$. If there exists some minimal pair of hyperplanes in $(\hyp{h},\hyp{k})$ which could be folded by an elementary fold, we fold them first, reducing the size of the set $(\hyp{h},\hyp{k})$ until there are no more minimal foldable hyperplanes. Then, the folding of $\hs{h}$ and $\hs{k}$ is an elementary folding which reduces the number of $G$-orbits of hyperplanes.

Now, we may assume that the map $f/G : \Hs{H}/G\to\Hs{H}'/G$ is injective. For each $G$-orbit of a hyperplane $G.\hyp{h}'$ in its image we fix a hyperplane $\hyp{h}'$ in $\Hs{H}'$ that belongs to this orbit and a finite set $S_{\hyp{h}'}$ of generators of the hyperplane stabilizer $\Stab_G{\hyp{h}'}$. We choose some representative $\hyp{h}\in\Hs{H}$ which is mapped by $f$ to $\hyp{h}'$. Let $c_{\hyp{h}'}$ be the number of generators in $S_{\hyp{h}'}$  that do not belong to $Stab_G(\hyp{h})$. Let $$c_f = \sum_{\hyp{h}'\in\Hs{H}'/G} c_{\hyp{h}'}$$ be the complexity of $f$.

We prove that if $c_f >0$ then by a finite sequence of elementary foldings one can reduce $c_f$. Let $\hyp{h}'$ be such that $c_{\hyp{h}'}>0$, and let $S_{\hyp{h}'}$ and $\hyp{h}$ be as in the definition of $c_{\hyp{h}'}$, and let $s\in S_{\hyp{h}'}$ be a generator of $\Stab_G (\hyp{h}')$ which does not belong to $\Stab_G (\hyp{h})$. Note that $f(\hyp{h})=f(s\hyp{h})$ thus by applying a similar procedure to the one above we perform elementary foldings until $\hyp{h}$ and $s\hyp{h}$ are folded. The stabilizer of the resulting hyperplane contains $s$ thus reduces the complexity by at least 1.

We complete the proof by observing that if $f/G$ is injective and $c_f=0$ then $f$ is an embedding of pocsets. 

\end{proof}
